Efficient Algorithms for Large-scale Generalized Eigenvector Computation and Canonical Correlation Analysis

This paper considers the problem of canonical-correlation analysis (CCA) (Hotelling, 1936) and, more broadly, the generalized eigenvector problem for a pair of symmetric matrices. These are two fundamental problems in data analysis and scientific computing with numerous applications in machine learning and statistics (Shi and Malik, 2000; Hardoon et al., 2004; Witten et al., 2009). We provide simple iterative algorithms, with improved runtimes, for solving these problems that are globally linearly convergent with moderate dependencies on the condition numbers and eigenvalue gaps of the matrices involved. We obtain our results by reducing CCA to the top-$k$ generalized eigenvector problem. We solve this problem through a general framework that simply requires black box access to an approximate linear system solver. Instantiating this framework with accelerated gradient descent we obtain a running time of $O(\frac{z k \sqrt{\kappa}}{\rho} \log(1/\epsilon) \log \left(k\kappa/\rho\right))$ where $z$ is the total number of nonzero entries, $\kappa$ is the condition number and $\rho$ is the relative eigenvalue gap of the appropriate matrices. Our algorithm is linear in the input size and the number of components $k$ up to a $\log(k)$ factor. This is essential for handling large-scale matrices that appear in practice. To the best of our knowledge this is the first such algorithm with global linear convergence. We hope that our results prompt further research and ultimately improve the practical running time for performing these important data analysis procedures on large data sets.

==> aux_proofs.tex <==
%!TEX root = main.tex

\section{Solving Linear System via Accelerated Gradient Descent}

 \begin{algorithm}[h!]
 \caption{Nesterov's accelerated gradient descent}\label{algo:AGD}
 \begin{algorithmic}
 \renewcommand{\algorithmicrequire}{\textbf{Input: }}
 \renewcommand{\algorithmicensure}{\textbf{Output: }}
 \REQUIRE $f$ which is $\alpha$-strongly convex and $\beta$-smooth, $Q = \beta/\alpha$, initial point $\x_0$, $T$.
 \ENSURE  minimizer $x^\star$ of $f$ .
 \FOR{$t = 0,\cdots,T-1$}
 \STATE $\y_{t+1} \leftarrow \x_t - (1/\beta)\cdot \grad f(\x_t)$
 \STATE $\x_{t+1} \leftarrow  \y_{t+1} +  (\sqrt{Q}-1)/(\sqrt{Q}+1) \cdot(\y_{t+1} - \y_t) $
 \ENDFOR
 \STATE \textbf{Return} $\y_T$.
 \end{algorithmic}
 \end{algorithm}
 \jccomment{state it in terms of learning rate $\eta$ and factor $Q$.}

\begin{theorem}[\cite{Nesterov1983}] \label{thm:AGD_guarantee}
	Let $f$ be $\alpha$-strongly convex and $\beta$-smooth, then accelerated gradient descent with learning rate $\eta = \frac{1}{\beta}$ and $\gamma = \frac{\sqrt{Q} - 1}{\sqrt{Q} + 1}$ satisfies: ($Q = \beta /\alpha$)
	\begin{equation}
	f(\x_t) - f(\x^\star) \le 2(f(\x_0) - f(\x^\star))\exp(-\frac{t}{\sqrt{Q}})
	\end{equation}
\end{theorem}

The following lemma specializes the above theorem for our setting of solving linear systems in a $d\times d$ PSD matrix $\B$.
\begin{lemma}\label{thm:NAG} Consider the function $f(\w) \defeq \frac{1}{2}\w\trans\B\w - \w\trans \z$, whose optimum is $\w^\star = \Binv \z$. Let $\epsilon_0 = 2 \left(f(\w_0) - f(\w^\star)\right) = \norm{\w_0 - \w^\star}_\B^2$. After $t \ge \sqrt{\cn(\B)} \log \frac{1}{\delta}$ iterations of accelerated gradient descent on $f(\w)$, we will have
	$\norm{\w_t - \w^\star}_\B^2 \le \delta \norm{\w_0 - \w^\star}_\B^2$. The runtime of the algorithm is $\Tcal{\delta} = \order{d^2 \sqrt{\cn(\B)} \log \frac{1}{\delta}}$.
\end{lemma}
\begin{proof}
	Clearly function $[\w\trans\B\w - \w\trans\A\w_t]$ is $\norm{\B}$-smooth and $\sigmin(\B)$-strongly convex.
	The global minimum of this function is when its gradient is equal to zero. That is:
	\begin{equation}
	\B\w^\star - \A \hat{\w} = 0 
	\end{equation}
	Moreover, for any point $\w$, we have:
	\begin{align}
	\norm{\w - \w^\star}^2_\B
	&= (\w - \w^\star)\trans \B (\w - \w^\star)
	= \w\trans \B \w - 2\w\trans \A \hat{\w} + \hat{\w}\trans \A\B^{-1}\A\hat{\w}\nn \\
	&= 2[f(\w) - f(\w^\star)]
	\end{align}
	Therefore, by directly applying Theorem \ref{thm:AGD_guarantee}, we finished the proof.
\end{proof}


==> related.tex <==
\subsection{Related Work}
